Quantum Levenberg--Marquardt Algorithm for optimization in Bundle Adjustment

In this paper we develop a quantum optimization algorithm and use it to solve the bundle adjustment problem with a simulated quantum computer. Bundle adjustment is the process of optimizing camera poses and sensor properties to best reconstruct the three-dimensional structure and viewing parameters. This problem is often solved using some implementation of the Levenberg--Marquardt algorithm. In this case we implement a quantum algorithm for solving the linear system of normal equations that calculates the optimization step in Levenberg--Marquardt. This procedure is the current bottleneck in the algorithmic complexity of bundle adjustment. The proposed quantum algorithm dramatically reduces the complexity of this operation with respect to the number of points. We investigate 9 configurations of a toy-model for bundle adjustment, limited to 10 points and 2 cameras. This optimization problem is solved both by using the sparse Levenberg-Marquardt algorithm and our quantum implementation. The resulting solutions are presented, showing an improved rate of convergence, together with an analysis of the theoretical speed up and the probability of running the algorithm successfully on a current quantum computer. The presented quantum algorithm is a seminal implementation of using quantum computing algorithms in order to solve complex optimization problems in computer vision, in particular bundle adjustment, which offers several avenues of further investigations.

==> HHL in LMA for Arxiv/ExtraResults.tex <==
\section{Additional results}

We present here the explicit results of the runs comparing LMA to the HHL. In Figs. 2-4 of the main text we see the performance of QLMA compared to the LMA with respect to an average across 9 different problems and the extremes of best and worse cases. That is, the problems that give highest or lowest cost at convergence of the algorithm. In Figure 5 of the main text, the comparison for one problem with setup 2 of damping parameters for both LMA and QLMA.

The quantum algorithm already converged mostly within the first 40 iterations, whereas the LMA did have a very hard time with the parameters of setup 1. When using setup 2 the LMA did considerably well, which can be seen in an example in Fig. 5 of the main text. Nonetheless, the HHL did show only modest improvements on convergence due to what we believe is the linear approximations employed in Trotter Suzuki expansion.

Here we show the cost convergence plots of all the problems under consideration and the results for the different setups. In the supplementary material is provided the optimization output for all problems. With a README.txt description on how to read the files. Each problem has been optimized with LMA with both setup 1 and setup 2 damping parameters, and with QLMA with only setup 1 damping parameters. One can see that for well constrained optimization landscapes like the 6th problem in Figs. \ref{fig:6a}, \ref{fig:6b} the QLMA offers no advantage to classical LMA, converging similarly at the beginning and being limited by the noise and approximations. On the other hand, challenging problems with difficult landscapes (like many of the problems under consideration in these examples) tend to take advantage of QLMA.

%%% ---- This problem that you proposed is not constrained, I tought you did something else. --- %
% In the test problem, not discussed in the main text, only a problem with two cameras and two points was considered. The cameras were left free only in one translational direction

% \begin{figure}[h!]
% \centering
% \includegraphics[width = 7.95cm]{lmahhlknown01}
% \caption{Comparison of the sparse LMA to QLMA which are stable, and 2 points, where we only one point is being moved with "noise" in the z-direction by 0.5, where the QLMA and LMA has the parameters as in setup 2 as in Table 2 of the main text. The sparse LMA is denoted by the orange line and the QLMA by the blue line}
% $\label{fig:small}
%\end{figure} 



\begin{figure}[h!]
\centering
\includegraphics[width = 0.45\textwidth]{lmahhl1}
\includegraphics[width = 0.45\textwidth]{lmahhl2}
\includegraphics[width = 0.45\textwidth]{lmahhl3}
\includegraphics[width = 0.45\textwidth]{lmahhl4}
\includegraphics[width = 0.45\textwidth]{lmahhl5}
\includegraphics[width = 0.45\textwidth]{lmahhl6}
\includegraphics[width = 0.45\textwidth]{lmahhl7}
\includegraphics[width = 0.45\textwidth]{lmahhl8}
\includegraphics[width = 0.45\textwidth]{lmahhl9}
\caption{Comparison of the sparse LMA to QLMA for the 9 random problems from setup 1 in Table 2 of the main text. The sparse LMA is denoted by the orange line and the QLMA by the blue line.}
\label{fig:6a}
\end{figure} 

\begin{figure}[h!]
\centering
\includegraphics[width = 0.45\textwidth]{lmahhl01_1}
\includegraphics[width = 0.45\textwidth]{lmahhl01_2}
\includegraphics[width = 0.45\textwidth]{lmahhl01_3}
\includegraphics[width = 0.45\textwidth]{lmahhl01_4}
\includegraphics[width = 0.45\textwidth]{lmahhl01_5}
\includegraphics[width = 0.45\textwidth]{lmahhl01_6}
\includegraphics[width = 0.45\textwidth]{lmahhl01_7}
\includegraphics[width = 0.45\textwidth]{lmahhl01_8}
\includegraphics[width = 0.45\textwidth]{lmahhl01_9}
\caption{Comparison of the sparse LMA to QLMA for the 9 random problems, where the QLMA has the parameters as in setup 1 and LMA as in setup 2 in Table 2 of the main text. The sparse LMA is denoted by the orange line and the QLMA by the blue line.}
\label{fig:6b}
\end{figure} 




==> HHL in LMA for Arxiv/TOYHHL.tex <==
% \documentclass[runningheads]{llncs}
% \usepackage{tikz}
% \usetikzlibrary{quantikz}
% \usepackage{xcolor}
% \usepackage{physics}
% \title{Trivial HHL example}
% \begin{document}

\section{HHL example}
\label{appendix:HHL}
Here we apply a simple analytical example of the HHL algorithm to explain each step of it. We additionally provide information regarding the relation with the HHL algorithm in general. Some steps become trivial due to the simplicity of the problem. For example, the decomposition of the unitary gates components for the QPE is not necessary. Therefore, no Trotter--Suzuki approximation is needed.
\newline
Let us assume we have the following problem,
\begin{align}
A x = b\Longleftrightarrow
\label{eq:linear}
    \begin{pmatrix}
    0&1\\
    1&0
    \end{pmatrix}
    \begin{pmatrix}
    y\\z
    \end{pmatrix}
    = \frac{1}{\sqrt{2}} \begin{pmatrix}
    1\\
    1
    \end{pmatrix}.
\end{align}
We could already make an educated guess that $x=y = 1/\sqrt{2}$ since $A^{-1}=A$. In general, one has to invert the matrix $A$ on the left, bring it onto the other side and solve it,
\begin{equation}
    \begin{pmatrix}
    y\\
    z
    \end{pmatrix}
    =    
    \begin{pmatrix}
    0&1\\
    1&0
    \end{pmatrix}^{-1}
    \frac{1}{\sqrt{2}} 
    \begin{pmatrix}
    1\\
    1
    \end{pmatrix},
\end{equation}
and classically the inversion of a general matrix is costly. How is this problem solved on a quantum computer using the HHL algorithm instead?

Quantum computers are built up by qubits, which are element of a two--dimensional Hilbert space that can be written in vector form as,
\begin{align}
\ket{0} = \begin{pmatrix}
1\\
0
\end{pmatrix},
\ket{1} = 
\begin{pmatrix}
0\\
1
\end{pmatrix}.
\end{align}
The quantum qubits are all connected by a tensor product.
\begin{figure}[h!]
\begin{quantikz}
\lstick{$\ket{0}$}&\qw\slice{1} &\qw\slice{2}&\qw\slice{3}&\qw\slice{4}&\gate{X}\gategroup[2,steps=1,style={dashed,
                   rounded corners, inner xsep=2pt},
                   background,label style={label position=above,anchor=
    north,yshift=0.5cm}]{{\sc INVERSION}}\slice{5}&\qw&\qw&\qw&\meter{}&\qw \\
\lstick{$\ket{0}$}&\qw &\gate{H}\gategroup[2,steps=3,style={dashed,
                   rounded corners, inner xsep=2pt},
                   background]{{\sc $QPE$}}&\ctrl{1}&\gate{H}&\octrl{-1}&\gate{H}\gategroup[2,steps=3,style={dashed,
                   rounded corners, inner xsep=2pt},
                   background]{{\sc $QPE^{\dagger}$}}&\ctrl{1}&\gate{H}&\meter{}&\qw\\
\lstick{$\ket{0}$}&\gate{H}&\qw&\gate{X}&\qw&\qw&\qw&\gate{X}&\qw&\qw&\qw
\end{quantikz}
\caption{Quantum computing operation can be represented as circuits, which can be seen here. The dashed lines just helps us as reference to explain each operational step. The explanation can be found in the text.}
\label{finalfigure}
\end{figure}

We set up a quantum circuit with three qubits, the first one is an ancilla register, which we will use later. Ancilla registers are additional qubits, needed to  implement algorithms. The second qubit is also an ancilla register which will be used for the QPE method and lastly the last qubit will encode the data.

We can apply operations onto such qubits (states) using unitary transformations called gates. For this example, we make mainly use of the quantum gate (operations) "Hadamard gate" and the flip gate X. 
Firstly, we are interested to encode our vector b in eq.(1) into the quantum computer. The Hadamard gate $H$ brings our state $\ket{0}$ to $1/\sqrt{2}(\ket{0}+\ket{1})$,
\begin{equation}
H = 
\frac{1}{\sqrt{2}}
    \begin{pmatrix}
    1&1\\
    1&-1
    \end{pmatrix}.
\end{equation}
We encode the data vector $\textbf{b}$ as $\ket{\psi} \equiv 1/\sqrt{2}(\ket{0}+\ket{1})$. Therefore, the total state of the computer becomes,
\begin{equation}
\label{colorequation}
 \begingroup\color{blue}\frac{1}{\sqrt{2}}\endgroup  (\ket{0}\ket{0}
\begingroup\color{blue}\ket{0}\endgroup
+\ket{0}\ket{0}\begingroup\color{blue}\ket{1}\endgroup) = \ket{0}\ket{0}\begingroup\color{blue}\ket{\psi}\endgroup,
\end{equation}
where the blue colored parts show the vector $\textbf{b}$, while the black $\ket{0}$s are unchanged ancilla qubits.
Then, we prepare our ancilla register of the QPE with a Hadamard gate. This results in the state that can be seen at step 2, 
\begin{equation}
    \frac{1}{\sqrt{2}}\ket{0}(\ket{0}+\ket{1})\ket{\psi}.
\end{equation}
Then we apply the control-X gate (CX).

The CX is a 2 qubit gate, and it is applied to 2 qubits simultaneously. The operation looks at the controlled qubit, which is seen in Fig. \ref{finalfigure} by a black dot. If it is $\ket{1}$ it applies an operation X onto the target register and performs a flip, which can be seen by a box with an X inside. In other words, X gate switches $\ket{1}$ to $\ket{0}$ and vice versa and the CX is given as,
\begin{equation}
\textrm{CX} = \begin{pmatrix}
1&0&0&0\\
0&1&0&0\\
0&0&0&1\\
0&0&1&0
\end{pmatrix}.
\end{equation}
Our CX gate is in the general a time evolution of our matrix and is a composition of arbitrary unitary operations, which can be carried on the quantum computer, as described in Eq.(4) in the main text. To apply the QPE we evaluate the time evolution in eq.(4) in the main text. $e^{-iAt}$, where A is Hermitian. $e^{-iAt}$ is unitary and can be expressed in gates. In our case the matrix A corresponds to the X gate and therefore our $e^{-iAt}$ is also implemented by an X gate. In general, the matrix $A$ and it's evolution $e^{-iAt}$ rarely have the same matrix representation and for this reason are decomposed and approximated using Trotter--Suzuki. The CX gate implements the Hamiltonian evolution $e^{iAt}$ if our control qubit is 1. A general evolution results in a the state at step 3,
\begin{equation}
    \frac{1}{\sqrt{2}}\ket{0}(\ket{0}+e^{2i\pi 0.\phi_1}\ket{1})\ket{\psi}.
\end{equation}
Here it can be seen that $\phi_1$ has to be 0 for the CX gate to obtain the correct results. This is because our solution is exact. Imagine we would have a non exact solution and the true value would lay between 0 and 1, then our $\phi_1$ would share a probability of being either in 0 and 1. With more ancilla qubits reserved for subsequent QPE measures it would be possible to get closer to an exact solution.

Notice that this control-gate can be a lot more complex, it can be that it is a composition of non commuting terms. In this case it would be necessary to apply the Trotter-Suzuki method, which is described in the main part of the paper.
Then after step 3 we apply another Hadamard gate, which acts as the inverse quantum Fourier transform, which makes it possible to write the exponent into a state. Additionally, $\ket{\psi}$ is a composition of the eigenvectors $\sum_j\ket{u_j}$ so we may straight write it as $\sum_j\ket{u_j}$.
\begin{equation}
   \sum_j \frac{1}{2}((1+e^{2\pi i 0.\phi_1})\ket{0}+(1-e^{2\pi i 0.\phi_1})\ket{1})\ket{0}\ket{u_j}.
\end{equation}
It can be noticed, as previously, that if $\phi_1=0$ then this results in,
\begin{equation}
     \frac{1}{2}((1+1)\ket{0}+(1-1)\ket{1})\ket{0}\ket{\psi} =\sum_j \lambda_j\ket{0}\ket{0}\ket{u_j},
\end{equation}
where $\lambda$ are the actual eigenvalues for the matrix for eigenvectors, which are both 1. %Note that usually we cannot find the eigenvalues that easily and it is required to use more ancilla gates, to get many different values between 0 and 1, then we can run the algorithm many times, and the state with the highest probability is encoding the most accurate value of the eigenvalues. Additionally, in those measurements we would need to measure the respective eigenvector to result in the corresponding eigenvalue in the QPE.

We can then take a further look into the final crucial stage of the HHL, which is the matrix inversion. The first qubit, which has been untouched so far, will be manipulated. In this problem this is again simplified because the inverse of $A$ is itself and due to $\lambda_j=1$, we have $1/\lambda_j$=$\lambda_j$. In general, we wish to move our first qubit to obtain,
\begin{equation}
    \sum_j\sqrt{1-\frac{C^2}{\lambda_j^2}}\ket{0}+\frac{C}{\lambda_j}\ket{1},
\end{equation}
where C is just a scalar between 0 and 1 obtained in the inversion, where in our case it is 1. $\lambda_j$ are generally the different eigenvalues, which in our case are both 1. Then we are interested in measuring $\ket{1}$, which holds the information of the inverse eigenvalues. Therefore the first qubit is being prepared with an Hadamard gate and then the matrix inversion is applied so that we result in the equation above.

In our case we can simply say if our second qubit is in the state $\ket{0}$, this is indicated by the circle between step 4 and 5 on the second qubit, which is the state with the information of our eigenvalues, then we rotate $\ket{0}$ to $\ket{1}$. 
%This may look as a really trivial move, because the probability of getting $\ket{1}$ is in our case 1, but generally it is a necessary step. 
At step 5, we therefore have.
\begin{equation}
    \sum_j \frac{1}{\lambda_j}\ket{0}\ket{1}\ket{u_j}.
\end{equation}
Then we are supposed to apply the QPE backwards to get rid of the QPE state $\ket{0}$ and the coefficient before, which in our case is only 1, this state then can be measured which concludes the circuit in Fig. \ref{finalfigure},
\begin{equation}
\label{final}
   \sum_j \lambda_j^{-1}\ket{u_j} = \frac{1}{\sqrt{2}}\left(\ket{0}+\ket{1}\right).
\end{equation}
And we can write $\ket{x} = \sum_j\lambda^{-1}_j\ket{u_j}$, which is exactly Eq.(\ref{final}) and solution to Eq. (\ref{eq:linear}). It may be noted again that $b$ in Eq.(\ref{eq:linear}) is decomposed into $\ket{u_j}$ on the quantum computer. Our final state encodes the solution desired.
Now the algorithm can be run an arbitrary number of times and the last qubit is measured this would give us a probability of measuring the probability 1/2 for each $\ket{0}$ and $\ket{1}$. The more often we run it the higher statistical probability we get to 1/2. Combining the results of the measurements gives us the full solution,
\begin{equation}
x = \begin{pmatrix}
y\\
z
\end{pmatrix}
=
\frac{1}{\sqrt{2}}\begin{pmatrix}
1\\
1
\end{pmatrix}.
\end{equation}
